Online convex optimization and no-regret learning: Algorithms, guarantees and applications

Spurred by the enthusiasm surrounding the "Big Data" paradigm, the mathematical and algorithmic tools of online optimization have found widespread use in problems where the trade-off between data exploration and exploitation plays a predominant role. This trade-off is of particular importance to several branches and applications of signal processing, such as data mining, statistical inference, multimedia indexing and wireless communications (to name but a few). With this in mind, the aim of this tutorial paper is to provide a gentle introduction to online optimization and learning algorithms that are asymptotically optimal in hindsight - i.e., they approach the performance of a virtual algorithm with unlimited computational power and full knowledge of the future, a property known as no-regret. Particular attention is devoted to identifying the algorithms' theoretical performance guarantees and to establish links with classic optimization paradigms (both static and stochastic). To allow a better understanding of this toolbox, we provide several examples throughout the tutorial ranging from metric learning to wireless resource allocation problems.

==> Algorithms/EXP3.tex <==
%----------------------------------------------------------------------
%%% EXP3 ALGORITHM
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


\begin{algorithmic}[1]
\REQUIRE
	parameter $\step>0$, mixing factor $\eps\in(0,1]$;
%\makeatletter
%\setcounter{ALC@line}{4}
%\makeatother
\STATE
	set $\score_{\pure} \leftarrow 0$ for each arm $\pure\in\pures$;
	\COMMENT{initialization}
\FOR{$\run=1$ \TO $\horizon$}
	\STATE
%		$\act \leftarrow \eps \cdot \unif + (1-\eps) \logit(\score)$;
		set $\act_{\pure} \leftarrow \eps/\nPures + (1-\eps) \logit_{\pure}(\score)$ for all $\pure\in\pures$;
		\COMMENT{strategy update}
	\STATE
		draw $\pure_{\run}$ according to $\act$;
		\COMMENT{arm selection}
	\STATE
		receive $\hat\pay_{\run} = \payv_{\run,\pure_{\run}}$;
		\COMMENT{receive reward}
	\STATE
		set $\hat\payv_{\pure} \leftarrow \hat\pay_{\run} \cdot \one(\pure_{\run} = \pure) / x_{\pure}$ for all $\pure\in\pures$;
		\COMMENT{estimate payoff vector}
	\STATE
		set $\score_{\pure} \leftarrow \score_{\pure} + \step \hat\payv_{\pure}$ for all $\pure\in\pures$;
		\COMMENT{score update}
\ENDFOR
\end{algorithmic}
